ReXCam: Resource-Efficient, Cross-Camera Video Analytics at Scale

Enterprises are increasingly deploying large camera networks for video analytics. Many target applications entail a common problem template: searching for and tracking an object or activity of interest (e.g. a speeding vehicle, a break-in) through a large camera network in live video. Such cross-camera analytics is compute and data intensive, with cost growing with the number of cameras and time. To address this cost challenge, we present ReXCam, a new system for efficient cross-camera video analytics. ReXCam exploits spatial and temporal locality in the dynamics of real camera networks to guide its inference-time search for a query identity. In an offline profiling phase, ReXCam builds a cross-camera correlation model that encodes the locality observed in historical traffic patterns. At inference time, ReXCam applies this model to filter frames that are not spatially and temporally correlated with the query identity's current position. In the cases of occasional missed detections, ReXCam performs a fast-replay search on recently filtered video frames, enabling gracefully recovery. Together, these techniques allow ReXCam to reduce compute workload by 8.3x on an 8-camera dataset, and by 23x - 38x on a simulated 130-camera dataset. ReXCam has been implemented and deployed on a testbed of 5 AWS DeepLens cameras.

==> introduction.tex <==
%\section{Introduction}

\jc{OLD INTRO}

Enterprises are increasingly deploying large camera networks for video analytics, for use cases ranging from public safety monitoring to patient oversight and business intelligence \cite{McKinsey}. For example, in Chicago, police access footage from 30,000 security cameras installed citywide to inform their responses to live crime reports \cite{ChicagoCam}. In London, police tap into 12,000 cameras installed on its underground transit network to identify and investigate threats to public safety \cite{LondonCCTV, UKCam}. In Paris, public hospitals plan to install 1,500 \textit{new} cameras to protect staff and monitor patients \cite{ParisCCTV}.

Close analysis of the live video from these deployments, however, remains a costly undertaking. Human monitoring does not scale to 1000s of cameras, and state-of-the-art neural networks are too expensive to operate on each video feed in real-time. In particular, at 1 Nvidia K80 GPU per video feed, automated analytics on the Chicago Public Schools' 7,000-camera deployment \cite{CPSCam} would require a \$28 million investment in GPU hardware, or cost \$6,300 per hour in GPU cloud time (about \$0.9 million per month) \cite{AzurePricing, EC2Pricing}, significant expenditures for a publicly-funded school system.

Recent work explores techniques to accelerate simple, per-frame tasks on single-camera video pipelines \cite{NoScope}, and support low-latency, after-the-fact queries on indexed, historical video \cite{Focus}. This work, however, does not address the key requirement of real video analytics applications: \textit{cross-camera analytics} on \textit{live} video. Multi-camera inference is the core capability that enables operators to monitor environments at scale, track and predict entity movement, and understand complex scenes, for applications such as flow control \cite{Genetec}, suspect tracking \cite{Optasia, Vigil}, and traffic management \cite{Optasia, VideoStorm}.

\begin{figure}
	\centering
	\includegraphics[width=0.90\columnwidth]{figures/abstract-new_cropped}
	\vspace{-3mm}
	\caption{\small ReXCam exploits a \textit{model of spatial and temporal correlations}, built on historical data, to reduce compute workload at inference time. In this figure, the camera network (on the y-axis) is plotted as per their mutual distances, e.g. c2 and c3 are spatially closer than c2 and c4. In searching for a query identity on c2 starting at $t$ (marked in dark red), ReXCam eliminates some cameras entirely (spatial filtering), and progressively searches first on c2 and c3 (but not c1 and c4), and then subsequently on c2, c3, c4 (but not c1). Also, it avoids searching in any of the cameras at times $t+2$ and $t+3$ (temporal filtering) because it knows that the traveling speed of the objects. The cameras and the times at which they are searched are marked with green lines, the rest represents compute savings.}
	\label{fig:overview}
	\vspace{-4mm}
\end{figure}

Cross-camera analytics, however, is compute and data intensive. Unlike simple, stateless tasks, such as object detection, cross-camera analytics entails discovering \textit{associations}, across frames and across cameras. Whereas cost grows linearly with time for per-frame queries, cost in cross-camera analytics also entails a second, spatial dimension -- the number of cameras in the network. For example, in the suspect tracking example, flagging frames containing an identified perpetrator requires searching both \textit{across} the camera network (which can span the entire city) and forward in time, at the throughput of the incoming video stream.

We can formalize the core problem here as follows: given a query instance of an object or entity of interest, we wish to return all subsequent instances of that identity in the live video, \textit{while examining as few video frames as possible}. We adopt the current practice as our baseline, which is to search every nearby camera for the query identity. This baseline is both extremely data intensive, and prone to a high rate of false positive matches -- by searching cameras indiscriminately, it encounters a large number of distractor instances, which derail inference \textit{precision} \cite{MSMT17}.

To address these severe cost and accuracy challenges, we present ReXCam -- a new system for efficient cross-camera video analytics. ReXCam exploits \textit{spatial} and \textit{temporal correlations} in large camera networks to reduce the size of the inference search space, and thus dramatically decrease compute cost. Spatial correlations indicate the degree of association between cameras -- the probability that a source camera will send traffic \textit{to} a particular destination camera. Temporal correlations indicate the degree of association between cameras \textit{over time} -- the probability that a source camera will send traffic to a particular destination camera \textit{at a particular time}. These correlations, learned offline on historical data, enable ReXCam to guide its inference-time search toward cameras and frames most likely to contain the query identity. In doing so, ReXCam is able to both substantially cut down its inference time workload, and increase its rate of true positive detections (see Figure \ref{fig:overview}).

ReXCam, at its core, represents a bridge between the physical properties in the physical world and capabilities of video analytics systems. Specifically, the spatio-temporal correlation represents a property of the physical space and it is applied to improve object tracking across multiple camera streams. To that end, there are three main challenges that arise. First, automatically obtaining spatio-temporal correlations is challenging on unlabeled video data, in addition to also being expensive for a vast camera network. Second, applying spatio-temporal correlations to existing object trackers is non-trivial and requires clean abstractions with the necessary resource-accuracy tradeoffs. Finally, any spatio-temporal profile is bound to have errors that will lead to missing of as well as spurious tracking of objects and we need a mechanism to detect and rectify such errors.

ReXCam operates in three phases. In an offline profiling phase, it constructs a \textit{cross-camera correlation model} on unlabeled video data, which encodes the locality observed in historical traffic patterns. This is an expensive one-time operation that requires assigning \textit{identifiers} to detected entities with an offline tracker, and then converting these identifiers into an aggregate profile of cross-camera correlations. At inference time, ReXCam uses this model to filter frames that are not spatially and temporally correlated to the query identity's current position, and thus unlikely to contain its next instance. On occasion, this pruning will cause ReXCam to miss query detections. In these cases, ReXCam performs a \textit{fast-replay search} on recently filtered frames, which uncovers the skipped query instances, and enables it to gracefully recover into its live cross-camera search.

Together these techniques enable significant improvements over the all-camera baseline. Evaluating on the well-known DukeMTMC dataset \cite{DukeMTMC}, which contains footage from 8 cameras located on the Duke University campus, we find that ReXCam is able to reduce compute cost by a factor of $4.6\times$ compared to the baseline, while improving precision (fraction of instances correct) by 27\%, at the price of just 1.6\% lower recall (fraction of instances found). Moreover, RexCam's fast-replay search scheme reduces delay by about 50\% relative to a scheme that searches for missed detections at the video frame rate. Finally, ReXCam is able to achieve these gains at a one-time offline profiling cost equal to running $600$ real-time queries, a fraction of the expected annual workload in many large video analytics operations \cite{VideoStorm, Vigil}.

We also evaluate our achieved savings factor relative to an oracle that could predict with certainty at inference time the destination camera for a given query instance. Such an oracle could achieve at maximum a $7.0\times$ workload reduction over the baseline on 8 cameras. In comparison, ReXCam, which is trained only on historical data, obtains a $4.6\times$ workload reduction, a substantial fraction of the oracle's gains.

==> introduction_junchen.tex <==
\section{Introduction}

%1st para: Start with the trend of more IoT devices and more real-time queries that use compute-intensive analytics. (also mention the growing accuracy of CNNs). A notable example is the enterprise-scale camera deployment.
The increasing proliferation of the Internet of Things (IoT) in building ``smart services'' has led to an explosion of data sources and applications that benefit from real-time {\em in-situ} inferences over these data. 
In parallel to this trend, the inference accuracy, especially for visual data, has been greatly improved, even surpassing the ``human level'', but at the expense of increased computing overhead.
These trends impose a tremendous challenge in how to live analyze these IoT data source {\em at scale}. 
When compared to internet web applications, the computational load of these application can be 100+$\times$~\cite{hauswald2015sirius}, and it is not limited by millions of human users, but rather the continuous activities of billions of sensors.

%2nd para: Analyzing the video feeds of a fleet of cameras is prohibitively expensive. The current 2nd para is good. 
In this work, we focus on {\em live video analytics on a network of cameras}, which embodies the key challenges of the aforementioned trend---{\em massive data sources}, {\em sheer volume}, and {\em compute-intensive inference logic} (\eg Convolutional Deep Neural Nets, CNNs) to achieve high accuracy.
Enterprises increasingly deploy large camera networks for use cases from public safety monitoring to patient oversight and business intelligence~\cite{McKinsey}.
For instance, Chicago and London police access footages from 30,000 and 12,000 cameras~\cite{ChicagoCam,LondonCCTV} respectively to response to crime reports in real time. 
However, human monitoring does not scale to 1000s of cameras, and state-of-the-art neural networks are too expensive to operate on each video feed in real-time. 
At 1 Nvidia K80 GPU per video feed, analyzing the Chicago Public Schools' 7,000-camera deployment~\cite{CPSCam} would require a \$28 million investment in GPU hardware, or cost \$6,300 per hour in GPU cloud time (about \$0.9 million per month) \cite{AzurePricing, EC2Pricing}, significant expenditures for a publicly-funded school system.

%3rd para: We argue the key reason for the high cost is that existing systems are built on same computing model of single edge-device pipeline. The current 3rd para talks focuses on cross-camera live video analysis, which probably is better placed in the 1st para.
We argue that key reason for the prohibitive computing cost is that existing systems are built on extending the computing model of {\em small} collections of edge devices (mostly a single device).
Recent work explores techniques to accelerate simple, per-frame tasks on single-camera video pipelines (\eg~\cite{NoScope}), and support low-latency, after-the-fact queries on indexed, historical video (\eg~\cite{Focus}). 
This work, however, does not address the requirements of live video analytics over a large fleet of cameras for {\em cross-camera analytics}---detecting and tracking query identities in the live streams across cameras over time. 
This is a key function behind many practical applications, \eg flow control~\cite{Genetec}, suspect tracking~\cite{Optasia, Vigil}, and traffic management~\cite{VideoStorm}.
Using the current practice as our baseline, one must search every nearby camera for the query identity, which not only needs a computing budget that grows linearly with the number of cameras, but also encounters a large number of distractor instances, derailing the inference precision~\cite{MSMT17}.

\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/abstract-new_cropped}
	\vspace{-3mm}
	\caption{\small ReXCam exploits a learned model of spatial and temporal correlations, built on historical data, to reduce compute workload at inference time. In this figure, the camera network (compressed to 1-D) is represented on the y-axis, and time on the x-axis. In searching for a query identity, ReXCam eliminates some cameras entirely (spatial filtering), and searches the others only within a narrow time window (temporal filtering).}
	\label{fig:overview}
	\vspace{-4mm}
\end{figure}

% This alternate caption is factually incorrect. ReXCam does not consider the travelling speed of objects at all.
ReXCam exploits a \textit{model of spatial and temporal correlations}, built on historical data, to reduce compute workload at inference time. In this figure, the camera network (on the y-axis) is plotted as per their mutual distances, e.g. c2 and c3 are spatially closer than c2 and c4. In searching for a query identity on c2 starting at $t$ (marked in dark red), ReXCam eliminates some cameras entirely (spatial filtering), and progressively searches first on c2 and c3 (but not c1 and c4), and then subsequently on c2, c3, c4 (but not c1). Also, it avoids searching in any of the cameras at times $t+2$ and $t+3$ (temporal filtering) because it knows that the traveling speed of the objects. The cameras and the times at which they are searched are marked with green lines, the rest represents compute savings.

%4th para: Our key insight is the cost of multi-camera analysis can be drastically reduced by exploring opportunities naturally arising from the {\em physical relationships} among the data sources (i.e., cameras). As a case study of this approach, this work explores the inherent {\em spatio-temporal correlations} to aggressively eliminate the frames to be processed. Explain the spatial & temporal correlations. Give some examples of how it works.
Our key insight is that the cost of cross-camera analysis can be drastically reduced by exploring opportunities naturally arising from the {\em physical-level correlations} among the data sources (\ie  cameras). To explore this approach, we develop {\em RexCam}, a cross-camera analytics system that leverages the inherent {\em spatio-temporal correlations} to aggressively prune the set of video frames to be processed, and thus dramatically decreases the compute cost.
Spatial correlations indicate the degree of association between cameras -- the probability that a source camera will send traffic \textit{to} a particular destination camera. Temporal correlations indicate the degree of association between cameras \textit{over time} -- the probability that a source camera will send traffic to a particular destination camera \textit{at a particular time}. These correlations, learned offline on historical data, enable ReXCam to guide its inference-time search toward cameras and frames most likely to contain the query identity. In doing so, ReXCam is able to both substantially cut down its inference time workload, and increase true positive detections (see Figure~\ref{fig:overview}).

%5th para: This paper presents RexCam, a concrete multi-camera analysis system that achieves an-order-of-magnitude saving in cost compared to existing approaches on the canonical application of spotlight search. 



%6th para: As RexCam bridges the analytics framework with the physical properties of the camera feeds, it naturally faces two challenges: (1) How to opportunistically maximize the benefits of using the spatio-temporal correlations without being affected by the noises typical to the physical-world properties? (2) How to extract useful spatio-temporal correlations from unlabeled video data? [Note I merged the 2nd and 3rd challenge in the draft]
As RexCam bridges the analytics framework with the cameras' physical properties, it naturally faces two challenges: (1) How to opportunistically maximize the benefits of using the spatio-temporal correlations without being affected by the noises typical to the physical-world properties? (2) How to extract useful spatio-temporal correlations from unlabeled video data? 



%7th para: A brief description of how RexCam works, i.e., the current 8th para
To address these challenges, ReXCam operates in three phases. In an offline profiling phase, it constructs a \textit{cross-camera correlation model} on unlabeled video data, which encodes the locality observed in historical traffic patterns. This is an expensive one-time operation that requires detecting entities with an offline tracker, and then converting them into an aggregate profile of cross-camera correlations. At inference time, ReXCam uses this model to filter frames that are not spatially and temporally correlated to the query identity's current position, and thus unlikely to contain its next instance. Occasionally, this pruning will cause ReXCam to miss query detections. In these cases, ReXCam performs a \textit{fast-replay search} on recently filtered frames, which uncovers the skipped query instances, and lets it to gracefully recover into its live video search.

%8th para: Eval summary, i.e., the current 9th & 10th para
%Together these techniques enable significant improvements over the all-camera baseline. 
We evaluated RexCam on the well-known DukeMTMC dataset \cite{DukeMTMC}, \jc{what about the other dataset?} which contains footage from 8 cameras located on the Duke University campus. 
We found that ReXCam is able to reduce compute cost by a factor of $4.6\times$ compared to the baseline, while improving precision (fraction of instances correct) by 27\%, at the price of just 1.6\% lower recall (fraction of instances found). Moreover, RexCam's fast-replay search scheme reduces delay by about 50\% relative to a scheme that searches for missed detections at the video frame rate. Finally, ReXCam is able to achieve these gains at a one-time offline profiling cost equal to running $600$ real-time queries, a fraction of the expected annual workload in many large video analytics operations \cite{VideoStorm, Vigil}.
Note that on a network of 8 cameras, the theoretical optimal cost saving factor would be $7\times$, \ie an {\em oracle} that knows in advance the destination camera for a given query instance. Thus, a cost saving of $4.6\times$ by RexCam shows it is promising in cutting the compute cost of large camera deployments.
%We also compared our achieved savings factor with that of an {\em oracle} that knows in advance the destination camera for a given query instance.
%Such an oracle could achieve at maximum a $7.0\times$ workload reduction over the baseline on 8 cameras. In comparison, ReXCam, which is trained only on historical data, obtains a $4.6\times$ workload reduction, a substantial fraction of the oracle's gains.


==> introduction_new.tex <==
\section{Introduction}

%1st para: Start with the trend of more IoT devices and more real-time queries that use compute-intensive analytics. (also mention the growing accuracy of CNNs). A notable example is the enterprise-scale camera deployment.
The increasing proliferation of the Internet of Things (IoT) has led to an explosion of data sources and applications that benefit from real-time inferences over these data. 
In parallel, the inference accuracy, especially for visual data, has greatly improved, even surpassing human levels, but at the expense of increased computing overhead. 
%These trends impose a tremendous challenge in how to live analyze these IoT data source {\em at scale}. 
%When compared to internet web applications, the computational load of these application can be 100+$\times$~\cite{hauswald2015sirius}, and it is not limited by millions of human users, but rather the continuous activities of billions of sensors.
%2nd para: Analyzing the video feeds of a fleet of cameras is prohibitively expensive. The current 2nd para is good. 
We believe that cameras are the most challenging of ``things'' in IoT and our focus is on {\em live video analytics on a network of cameras}, which embodies the key challenges of the aforementioned trends---{\em massive data sources}, {\em sheer volume}, and {\em compute-intensive inference logic} (\eg Convolutional Deep Neural Nets, CNNs) to achieve high accuracy.
Enterprises increasingly deploy large camera networks for use cases from public safety monitoring to patient oversight and business intelligence~\cite{McKinsey}.
For instance, Chicago and London police access footages from 30,000 and 12,000 cameras~\cite{ChicagoCam,LondonCCTV} respectively to response to crime reports in real time. 
However, state-of-the-art neural networks are too expensive to operate on each video feed in real-time. 
%At 1 Nvidia K80 GPU per video feed, analyzing the Chicago Public Schools' 7,000-camera deployment~\cite{CPSCam} would require a \$28 million investment in GPU hardware, or cost \$6,300 per hour in GPU cloud time (about \$0.9 million per month) \cite{AzurePricing, EC2Pricing}, significant expenditures for a publicly-funded school system.

Recent work explores techniques to accelerate analytics on live videos as well as for indexing historical videos. Techniques include frame sampling and downsizing for resource-accuracy tradeoffs \cite{VideoStorm, awstream, Chameleon}, using compressed and specialized models \cite{Focus}, and designing cascaded filters for early discard of frames \cite{NoScope}. However, in all these techniques, the inference optimization of each video stream's analytics is {\em independent} of the optimizations on the other streams. % {\em single-camera} video pipelines (\eg~\cite{NoScope}), and support after-the-fact queries on indexed, historical video (\eg~\cite{Focus}). 

%3rd para: We argue the key reason for the high cost is that existing systems are built on same computing model of single edge-device pipeline. The current 3rd para talks focuses on cross-camera live video analysis, which probably is better placed in the 1st para.
%We argue that key reason for the prohibitive computing cost is that existing systems are built on extending the computing model of {\em small} collections of edge devices (mostly a single device).
Such single-camera optimizations do not address the requirements of {\em cross-camera video analytics} over a large fleet of cameras, i.e., detecting and tracking a query ``identity'' in the live streams as the queried identity moves {\em across cameras over time}. Cross-camera analytics is a key primitive behind many high-value applications in practice, \eg crowd control~\cite{Genetec}, suspect tracking~\cite{Optasia, Vigil}, and traffic management~\cite{VideoStorm}. Cross-camera analytics is compute and data intensive. Unlike stateless tasks, such as object detection, cross-camera analytics entails discovering \textit{associations}, across frames and across cameras. 
%Whereas cost grows linearly with time for per-frame queries, cost in cross-camera analytics also entails a second, spatial dimension -- the number of cameras in the network (e.g., in the city), thus limiting the efficacy of techniques that optimize each camera's stream analytics standalone.% For example, in the suspect tracking example, flagging frames containing an identified perpetrator requires searching both \textit{across} the camera network (which can span the entire city) and forward in time, at the throughput of the incoming video stream.
Using the current practice of (optimized) single-camera analytics as our baseline, one must still search a large number of nearby cameras for the query identity, which not only grows the computing cost linearly with the number of cameras, but also leads to many ``distractor'' instances that derails the inference precision~\cite{MSMT17}.

\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/abstract-new_cropped}
	\vspace{-3mm}
	\caption{\small ReXCam exploits a learned model of spatial and temporal correlations, built on historical data, to reduce compute workload at inference time. In this figure, the camera network (compressed to 1-D) is represented on the y-axis, and time on the x-axis. In searching for a query identity, ReXCam eliminates some cameras entirely (spatial filtering), and searches the others only within a narrow time window (temporal filtering).}
	\label{fig:example}
	\vspace{-4mm}
\end{figure}

% NOTE: This caption is factually incorrect. ReXCam does not consider the traveling speed of objects at all. Also, the ellipses do NOT represent skipped time windows. Please consult the original figure.
% \caption{\small ReXCam exploits a
% \textit{spatio-temporal correlations} to reduce compute workload at inference time. The camera network (on the y-axis) is plotted according to their mutual distances, e.g. c2 and c3 are spatially closer than c2 and c4. In searching for a query identity on c2 starting at $t$ (marked in dark red), ReXCam eliminates some cameras entirely (spatial filtering), and progressively searches first on c2 and c3 (but not c1 and c4), and then subsequently on c2, c3, c4 (but not c1). Also, it avoids searching in any of the cameras at times $t+2$ and $t+3$ (temporal filtering) because it knows the traveling speed of the objects. The cameras and the times at which they are searched are marked with green lines, the unmarked portions represent compute savings.}

%4th para: Our key insight is the cost of multi-camera analysis can be drastically reduced by exploring opportunities naturally arising from the {\em physical relationships} among the data sources (i.e., cameras). As a case study of this approach, this work explores the inherent {\em spatio-temporal correlations} to aggressively eliminate the frames to be processed. Explain the spatial & temporal correlations. Give some examples of how it works.
Our key insight is that the cost of cross-camera analysis can be drastically reduced by exploring opportunities naturally arising from the {\em physical correlations} among the data sources (\ie  cameras). We develop ReXCam, a cross-camera analytics system that leverages the inherent {\em spatio-temporal correlations} to aggressively prune the set of video frames to be processed, and thus dramatically decreases the compute cost.
Spatial correlations indicate the degree of association between cameras -- the probability that a source camera will send traffic \textit{to} a particular destination camera. Temporal correlations indicate the degree of association between cameras \textit{over time} -- the probability that a source camera will send traffic to a particular destination camera \textit{at a particular time}. These correlations, learned offline on historical data, enable ReXCam to guide its inference-time search toward cameras and frames most likely to contain the query identity. By doing so, ReXCam substantially cuts down inference workload, and increases true positive detections (see Figure~\ref{fig:example}).

%5th para: This paper presents RexCam, a concrete multi-camera analysis system that achieves an-order-of-magnitude saving in cost compared to existing approaches on the canonical application of spotlight search. 



%6th para: As RexCam bridges the analytics framework with the physical properties of the camera feeds, it naturally faces two challenges: (1) How to opportunistically maximize the benefits of using the spatio-temporal correlations without being affected by the noises typical to the physical-world properties? (2) How to extract useful spatio-temporal correlations from unlabeled video data? [Note I merged the 2nd and 3rd challenge in the draft]
As RexCam bridges the analytics on videos with the cameras' physical properties, it faces two challenges: (a) How to maximize the benefits of using the spatio-temporal correlations while coping with the noises typical to the physical-world? (b) How to extract useful spatio-temporal correlations from unlabeled video data? 



%7th para: A brief description of how RexCam works, i.e., the current 8th para
To address these challenges, ReXCam operates in three phases. 1) In an offline profiling phase, it constructs a \textit{cross-camera correlation model} on unlabeled video data, which encodes the locality observed in historical traffic patterns. This is an expensive one-time operation that requires detecting entities with an offline tracker, and then converting them into an aggregate profile of cross-camera correlations. 2) At inference time, ReXCam uses this model to filter frames that are not spatially and temporally correlated to the query identity's current position, and thus unlikely to contain its next instance. 3) Occasionally, this pruning will cause ReXCam to miss query detections. In these cases, ReXCam performs a \textit{fast-replay search} on recently filtered frames, which uncovers the skipped query instances, and lets it to gracefully recover into its live video search.

%8th para: Eval summary, i.e., the current 9th & 10th para
%Together these techniques enable significant improvements over the all-camera baseline. 
We evaluated RexCam on the well-known DukeMTMC dataset \cite{DukeMTMC}, \jc{what about the other dataset?} which contains footage from 8 cameras located on the Duke University campus. 
We found that ReXCam is able to reduce compute cost by a factor of $4.6\times$ compared to the baseline, while improving precision (fraction of instances correct) by 27\%, at the price of just 1.6\% lower recall (fraction of instances found). Moreover, RexCam's fast-replay search scheme reduces delay by about 50\% relative to a scheme that searches for missed detections at the video frame rate. Finally, ReXCam is able to achieve these gains at a one-time offline profiling cost equal to running $600$ real-time queries, a fraction of the expected annual workload in many large video analytics operations \cite{VideoStorm, Vigil}.
Note that on a network of 8 cameras, the theoretical optimal cost saving factor would be $7\times$, \ie an {\em oracle} that knows in advance the destination camera for a given query instance. Thus, a cost saving of $4.6\times$ by RexCam shows it is promising in cutting the compute cost of large camera deployments.
%We also compared our achieved savings factor with that of an {\em oracle} that knows in advance the destination camera for a given query instance.
%Such an oracle could achieve at maximum a $7.0\times$ workload reduction over the baseline on 8 cameras. In comparison, ReXCam, which is trained only on historical data, obtains a $4.6\times$ workload reduction, a substantial fraction of the oracle's gains.


==> operation.tex <==
%!TEX root = main.tex

\section{ReXCam Tracking Pipeline}
\label{sec:pipeline}

We describe the design of ReXCam by firstly introducing the tracking pipeline. 

\subsection{Identity re-identification}

Identity tracking in ReXCam is implemented on a basic computer vision primitive known as \textit{identity re-identification}. Given an image of a query identity $q$, a re-identification (re-id) algorithm ranks every image $g_i$ in a gallery $G$ based on its \textit{feature distance} to $q$ -- a Euclidean distance metric defined on the space $R^{1 \times h \times w \times c}$ of image features (see \textbf{Figure \ref{fig:re-id}}). Typically, these features are the intermediate representation of a deep neural network trained to associate instances of the same (co-identical) entity, and differentiate instances of different (non-co-identical) entities.

A successful re-id algorithm will rank co-identical (positive) instances to the query more highly in the list than non-co-identical (negative) instances. By extension, in a \textit{perfect} re-id ranking, all $i$ co-identical instances to $q$ present in $G$ appear in the top $i$ list entries. Over the full set of queries $q \in Q$, a perfect ranking satisfies:
\begin{align}
\forall q \in Q \quad \max_{p \sim q} d(q, p) < \min_{n \nsim q} d(q, n)
\end{align}
where $d(\cdot, \cdot)$ denotes the feature distance metric, $p$ denotes positive instances, and $n$ negative instances \cite{DukeFeatures}.

\begin{figure}
	\includegraphics[width=0.48\textwidth]{re-identification}
	\vspace{-6mm}
	\caption{Illustration of identity re-identification.}
	\label{fig:re-id}
	\vspace{-4mm}
\end{figure}

A re-id ranking is typically evaluated on two metrics. The first is \textit{rank-$k$ accuracy}, which is the percentage of the top $k$ list entries that consist of positive examples. Rank-$1$ accuracy, for example, indicates how often the top ranked entry in the gallery matches the query. The second metric is \textit{mean average precision} (mAP). mAP is a finer-grained accuracy metric from information retrieval and computer vision that sums the product of (a) precision and (b) change in recall across every position in the ranking. \ys{Is mAP the average of the maximum precisions at different recall values?} Both rank-$k$ accuracy and mAP values fall between 0\% and 100\%, where 100\% indicates a perfect ranking.

Person re-identification is considered a challenging problem in computer vision. In general, low-resolution images, uniform clothing patterns, and stark differences in lighting or viewpoint across cameras -- characteristics of difficult datasets -- all conspire to reduce ranking accuracy \cite{MSMT17}.

\subsection{Identity tracking}

Given the ability to rank a set of detections based on their similarity to a query image, we can now define and implement \textit{cross-camera identity tracking}. In tracking, the input consists of a query image $q$, extracted from frame $f_q$ on camera $c_q$ where $q$ was last seen. The goal is to flag all subsequent frames, on all cameras, that contain co-identical instances to $q$, while maximizing two metrics: (1) recall -- the fraction of positive instances successfully retrieved, and (2) precision -- the fraction of retrieved instances that are positive. Note that $q$ can appear again on the same camera ($c = q^c$), different cameras ($c \neq q^c$), or else exit the network altogether at any point. Tracking stops when $q$ has deemed to have exited.

\begin{algorithm}
	\caption{Tracking in ReXCam.}
	\label{alg:tracking}
	\begin{algorithmic}[1]
		% \scriptsize
		\State \textbf{input}: video feeds $\{V_c\}$ for camera $c$
		\For{query $(q, f_q, c_q) \in Q$}
		\State $q_{\text{feat}} = \text{features}(q)$ \Comment{extract image features}
		\State $f_{\text{curr}} = f_q + 1$ \Comment{init current frame index}
		\State $M_q = []$ \Comment{init query match array}
		\While{$(f_{\text{curr}} - f_q) \leq \text{exit\_t}$}
		\State $\text{frames} = \text{get\_frames}(V, f_{\text{curr}})$
		\State $\text{gallery} = \text{extract\_entities}(\text{frames})$
		\State $\text{ranked} = \text{rank\_reid}(q_{\text{feat}}, \text{gallery})$
		\If{ $\text{ranked}[0][\text{dist}] < \text{match\_thresh}$}
		\State $M_q = \text{append}(M_q, \text{ranked}[0][\text{img}])$
		\State $q_{\text{feat}} = \text{update\_rep}(q_{\text{feat}}, \text{ranked}[0][\text{feat}])$
		\State $f_q = f_{\text{curr}}$
		\EndIf
		\State $f_{\text{curr}} = \text{increment}(f_{\text{curr}})$
		\EndWhile
		\EndFor
		\State \textbf{output}: matched detections $\{M_q\}$
	\end{algorithmic}
\end{algorithm}

We propose \textbf{Algorithm \ref{alg:tracking}} for cross-camera identity tracking. Given a set of video feeds $V_c$, we wish to execute $|Q|$ separate tracking queries. For each tracking query $q$, we begin by extracting image features $q_{\text{feat}}$ and initializing an empty array of discovered matches $M_q$. We then proceed to repeatedly: (1) retrieve the current frame from each video feed, (2) extract entities from each frame using an object detection model, (3) rank the detections based on their feature distance to $q$ using a re-id model, and (4) check if the distance to the top ranked detection is within a \textit{match threshold}.

The match threshold is a binary decision cutoff we impose to convert re-id, a ranking algorithm, into a \textit{classifier}. In particular, since it is possible for $q$ to fail to appear in \textit{any} camera at a given frame index $f_\text{curr}$ (due to occlusions, blind spots in the camera network), the detection gallery may contain no co-identical instances. Thus, we must determine if the top match is in fact co-identical. If we decide that it is, we add the detection to our array of matches $M_q$, update our query \textit{representation} $q_{\text{feat}}$ to incorporate the features of the new instance of $q$ \ys{details of representation update?}, update the query frame index $f_q$ to $f_{\text{curr}}$, and proceed with tracking $q$ on the same camera. If we instead decide that no co-identical instances are present at $f_\text{curr}$, we increment the current frame index $f_\text{curr}$, and proceed to search the next set of frames for $q$.

We continue searching until the gap between the last detected instance of $q$ and our current frame index exceeds a pre-defined \textit{exit threshold} (defined as $\text{exit\_t}$ in Algorithm \ref{alg:tracking}). At this point, we conclude that $q$ must have exited the camera network, and cease tracking $q$. We then repeat this process for the next query in $Q$.


\section{Spatio-temporal correlations}
Based on tracking pipeline in SEction~\ref{sec:pipeline}, we now describe how to leverage spatio-temporal correlations to improve cost efficiency and inference accuracy in multi-camera video analytics.

\subsection{Overview}
ReXCam exploits two forms of cross-camera correlations. \textbf{Spatial correlations} capture long-term associations between camera pairs. These include, but are not limited to, associations arising from camera topology (e.g. nearby cameras tend to send more traffic to each other than distant cameras). The degree of spatial correlation $d_{sc}$ between two cameras $c_s, c_d$ is quantified by the ratio of (a) the number of entities leaving the source camera for the destination camera, $n(c_s, c_d)$, to (b) the total number of entities leaving the source camera:
\begin{align}
	d_{sc}(c_s, c_d) = \frac{n(c_s, c_d)}{\sum_i n(c_s, c_i)}
\end{align}
In particular, a camera $c_i$ that receives a large fraction of the outgoing traffic from source camera $c_s$ is said to be \textit{highly correlated} to camera $c_s$. Note that spatial correlations may be asymmetric. In the previous example, it is possible that camera $c_s$ is \textit{not} highly correlated with camera $c_i$, even if the converse is true. ReXCam exploits spatial correlations in its search for a query identity $q$ by prioritizing destination cameras that are highly correlated to the query camera $c_q$.

\textbf{Temporal correlations} capture associations between camera pairs \textit{over time}. If a large percentage of the traffic leaving camera $c_s$ for camera $c_d$ arrives between $t_1$ and $t_2$, then camera $c_d$ is said to be \textit{highly correlated in $[t_1, t_2]$} to camera $c_s$. The degree of temporal correlation $d_{tc}$ between two cameras $c_s, c_d$ during a time interval $[t_1, t_2]$ is quantified by the ratio of (a) entities reaching $c_d$ from $c_s$ during $[t_1, t_2]$ to (b) total entities reaching $c_d$ from $c_s$:
\begin{align}
	d_{tc}(c_s, c_d, [t_1, t_2]) = \frac{n(c_s, c_d, [t_1, t_2])}{n(c_s, c_d)}
\end{align}
Like spatial correlations, temporal correlations can be asymmetric, with arrival counts peaking at different time intervals in the different directions. Note also that camera $c_d$ can be temporally correlated to $c_s$ at time $t$, without $c_d$ being \textit{spatially} correlated to $c_s$, if most of the small amount of traffic from $c_s$ to $c_d$ arrives around $t$. ReXCam exploits temporal correlations in its search for $q$ by prioritizing the \textit{time window} $[t_1, t_2]$ in which a destination camera is most correlated with the query camera $c_q$.

\subsection{Spatio-temporal model} \label{sec:model}

Given a source camera $c_s$, the current frame index $f_{\text{curr}}$, which serves as a timestamp, and a destination camera $c_d$, our proposed spatio-temporal model $M$ outputs \texttt{true} if $c_d$ is both spatially correlated and temporally correlated with $c_s$ at $f_{\text{curr}}$, and \texttt{false} otherwise.

The thresholds for being spatially correlated with $c_s$, and temporally correlated with $c_s$ at time $f_{\text{curr}}$, are model parameters that are set by the system operator. As an example, we may first wish to search cameras receiving at least $s_{\text{thresh}} = 5\%$ of traffic from $c_s$, during the time window containing the first $1 - t_{\text{thresh}} = 98\%$ of traffic from $c_s$. These parameter settings exclude both \textit{outlier cameras} (cameras receiving less than $5\%$ of the traffic from $c_s$) and \textit{outlier frames} (frames containing either the last 2\% of the traffic from $c_s$, or no traffic from $c_s$).

Once built, $M$ will only output \texttt{true} (i.e. 1) if both conditions $s_{\text{thresh}}$ and $t_{\text{thresh}}$ are met at $f_{\text{curr}}$. Formally:
\begin{align}
M(c_s, c_d, f_{\text{curr}})& = \label{eq:model}
	\begin{cases}
		1, & d_{sc}(c_s, c_d) \geq s_{\text{thresh}}\\
		& \quad \textbf{and} \\
		& d_{tc}(c_s, c_d, [f_0, f_\text{curr}]) \leq 1 - t_{\text{thresh}}\\
		0, & \text{otherwise}
	\end{cases}
\end{align}
Here $f_0$ is the frame index at which the first historical arrival at $c_d$ from $c_s$ was recorded. Our temporal filter checks if the volume of historical traffic that arrived at $c_d$ between $[f_0, f_\text{curr}]$ is less than $1 - t_{\text{thresh}}$\% of the total traffic. This ensures that $f_\text{curr}$ falls in the ``dense'' part of the travel time distribution, where we are likely to find $q$. (Note that we must also check that $f_\text{curr} \geq f_0$).

Our model $M$ encodes the spatial and temporal locality inherent in the camera network (see Section \ref{sec:empirical}). By first examining spatio-temporally correlated camera frames, we explore the part of the inference space most likely to contain $q$. A ``cache hit'' reduces inference cost, as we avoid searching the entire space of detections at $f_\text{curr}$. On the other hand, on a ``cache miss'', we must subsequently process the remainder of the inference space. On these rarer cache misses, using $M$ incurs a penalty, as this procedure introduces \textit{delay}: instead of detecting $q$ in real-time, we must find $q$ in past video frames in our second pass through video feed $V$. If cache misses are rare enough, and we can mitigate the delay they introduce (Section \ref{sec:replay}), then such a system will outperform one that is locality-agnostic.


\subsection{Applying the model}
\label{subsec:inference}

Applying such a spatio-temporal model involves a series of modifications to the cross-camera tracking pipeline (see \textbf{Algorithm \ref{alg:tracking-st}}). First, in addition to the video feeds $\{V_c\}$, we must pass as input the spatio-temporal model itself. The model is represented as two filters, both of which return \{\texttt{true}, \texttt{false}\} values: (1) $\textbf{spatial\_corr}(c_s, c_d)$, which given a source camera $c_s$ and a destination camera $c_d$ returns \texttt{true} if $c_d$ is correlated with $c_s$, and (2) $\textbf{temporal\_corr}(c_s, c_d, f)$, which given a source camera $c_s$, a destination camera $c_d$, and a frame index $f$, returns \texttt{true} if $c_d$ is correlated with $c_s$ at $f$. At query time, these two functions are passed to a higher-order \textbf{filter} function, which given a list of video feeds $V$, returns the subset of cameras in $V$ that are \textit{both} spatially and temporally correlated to $c_q$ at $f_{\text{curr}}$.

Applying \textbf{filter} reduces the inference search space, at each frame step $f_{\text{curr}}$, from all entity detections at $f_{\text{curr}}$ on every camera to all entity detections at $f_{\text{curr}}$ on \textit{correlated} cameras. This allows us to abstain from running object detection and feature extraction models on non-correlated cameras, and reduces the size of the re-id gallery in the ranking step.

\begin{algorithm}
	\caption{Tracking with the spatio-temporal model}
	\label{alg:tracking-st}
	\begin{algorithmic}[1]
		% \scriptsize
		\State \textbf{input}: video feeds $\{V_c\}$ for camera $c$,
		\\ \quad\quad\quad $\text{spatial\_corr}(c_s, c_d) \rightarrow \{\texttt{true}, \texttt{false}\} $
		\\ \quad\quad\quad $\text{temporal\_corr}(c_s, c_d, f) \rightarrow \{\texttt{true}, \texttt{false}\} $
		\For{query $(q, f_q, c_q) \in Q$}
		\State $q_{\text{feat}} = \text{features}(q)$ \Comment{extract image features}
		\State $f_{\text{curr}} = f_q + 1$ \Comment{init current frame index}
		\State $M_q = []$ \Comment{init query match array}
		\State $\text{phase} = 1$ \Comment{start phase one}
		\While{$(f_{\text{curr}} - f_q) \leq \text{exit\_t}$}
		\State $V_{\text{corr}} = \textbf{filter}(\text{sp\_corr}, \text{tp\_corr}, c_q, f_{\text{curr}}, V)$
		\State $\text{frames} = \text{get\_frames}(V_{\text{corr}}, f_{\text{curr}})$
		\State $\text{gallery} = \text{extract\_entities}(\text{frames})$
		\State $\text{ranked} = \text{rank\_reid}(q_{\text{feat}}, \text{gallery})$
		\If{ $\text{ranked}[0][\text{dist}] < \text{match\_thresh}$}
		\State $M_q = \text{append}(M_q, \text{ranked}[0][\text{img}])$
		\State $q_{\text{feat}} = \text{update\_rep}(q_{\text{feat}}, \text{ranked}[0][\text{feat}])$
		\State $f_q = f_{\text{curr}}$
		\State $\text{phase} = 1 \ys{break?}$ \Comment{reset to phase one}
		\EndIf
		\State $f_{\text{curr}} = \text{increment}(f_{\text{curr}})$
		\If{$\text{phase} = 1 \textbf{ and } (f_{\text{curr}} - f_q) > \text{exit\_t}$}
		\State $f_{\text{curr}} = f_q + 1$ \Comment{reset frame index}
		\State $\text{sp\_corr} = \neg\text{sp\_corr}$ \Comment{invert spatial filter}
		\State $\text{phase} = 2$ \Comment{start phase two}
		\EndIf
		\EndWhile
		\EndFor
		\State \textbf{output}: matched detections $\{M_q\}$
	\end{algorithmic}
\end{algorithm}

The penalty paid for this reduced compute cost is missed true positive detections. While we expect instances of $q$ to appear on correlated cameras at peak times \textit{in general}, we also expect occasions where this will not be the case. When $q$ reappears on non-correlated cameras or at non-peak times, we will fail to rediscover $q$, and at $f_{\text{curr}} = f_q + \text{exit\_t}$, incorrectly declare that $q$ has exited. To address this issue, we introduce a conditional second phase to Alg. \ref{alg:tracking-st}, which we call \textit{replay search}. Given no matches on the correlated cameras from $f_{\text{curr}} = f_q + 1$ to $f_{\text{curr}} = f_q + \text{exit\_t}$, we regress to searching the cameras \textit{not} correlated with $c_q$. \ys{ReXCam doesn't save anything on traffic that exits the network. Any numbers to show this is not significant?} One way to implement this is to negate the output of the correlation filter $\textbf{spatial\_corr}(c_s, c_d)$, and instead filter the cameras in $V$ that we have \textit{already searched}.

In particular, phase two of Alg. \ref{alg:tracking-st} (lines 21-24) initiates when we cross the exit threshold ($\text{exit\_t}$), which signifies that either we have missed $q$ by pruning the search space, or that $q$ has in fact exited the camera network. To rule out the former possibility, we reset $f_{\text{curr}}$ to the query frame index $f_q$, and invert our spatial correlation filter $\textbf{spatial\_corr}(c_s, c_d)$. We then restart the tracking procedure from $f_{\text{curr}} = f_q + 1$, looking for the next instance of $q$ in video feeds \textit{not} spatially correlated with $c_q$. If we do discover an instance of $q$, we proceed with tracking from that detection, initiating a new phase one. If we do not, then we cease our search for $q$ at the exit threshold, as in the original algorithm (Alg. \ref{alg:tracking}).

Note that regressing to the baseline involves searching for $q$ in \textit{historical video}. Doing this efficiently, and mitigating the delay we accumulate by searching for $q$ in the past, while the live video stream progresses, is a key challenge introduced by spatio-temporal filtering. We discuss our solution, a fast-replay search mode, in \S\ref{sec:replay}.

\subsection{Cost savings}
\label{sec:cost-savings}
We can quantify the savings achieved by spatio-temporal filtering, compared to a baseline that applies no filtering and thereby searches all cameras, with the following cost ratio:
\begin{align}
r_c &= \frac{\text{c}_{\text{baseline}}^{\text{det}} + \text{c}_{\text{baseline}}^{\text{feat}}  + \text{c}_{\text{baseline}}^\text{reid}}{\text{c}_{\text{st-filter}}^{\text{det}} + \text{c}_{\text{st-filter}}^{\text{feat}}  + \text{c}_{\text{st-filter}}^\text{reid}} \\[+12pt]
&= \frac{\text{c}^{\text{det}}|V| + \text{c}^{\text{feat}}|V|\cdot \bar d + \text{c}^{\text{reid}}|V|\cdot \bar d}{\text{c}^{\text{det}}|V_{\text{corr}}| + \text{c}^{\text{feat}}|V_{\text{corr}}|\cdot \bar d + \text{c}^{\text{reid}}|V_{\text{corr}}|\cdot \bar d} \\[+12pt]
&= \frac{|V|}{|V_{\text{corr}}|} \label{eq:ratio}
\end{align}
where $|V|$ refers to the total number of cameras, $|V_{\text{corr}}|$ the number of cameras correlated with the query camera $c_q$ at $f_{\text{curr}}$, and $\bar d$ the average number of entity detections per camera frame, while $\text{c}^{\text{det}}$, $\text{c}^{\text{feat}}$, $\text{c}^{\text{re-id}}$ represent the costs of running object detection, extracting features, and computing re-id feature distance to $q$, respectively, for a single frame or detection (see Algorithm \ref{alg:tracking}). Equation \ref{eq:ratio} signifies that the achieved savings factor $r_c$ reduces to the ratio of (a) the total number of cameras $|V|$ and (b) the number of correlated cameras $|V_{\text{corr}}|$ at a given frame step. While $|V_{\text{corr}}|$ varies based on $c_q$ and $f_{\text{curr}}$, we see that, on average, achieved savings are proportional to the degree of correlation filtering.

==> relatedwork_old.tex <==
%!TEX root = main.tex

\section{Related Work}

\noindent{\bf Systems for Video Analytics.} Since 2016, a sizable body of work on video analytics has emerged in the systems and data management community. We briefly survey five key papers. Optasia parallelizes video query plans and de-duplicates the work of common modules (e.g. background subtraction) in a dataflow framework to improve query completion time and reduce resource usage \cite{Optasia}. VideoStorm investigates the variance in quality-lag requirements between common video analytics queries (e.g. scanning license plates for billing on toll routes vs. issuing AMBER Alerts), and proposes an offline profiler and online scheduler for their optimal execution \cite{VideoStorm}. NoScope accepts specialized queries (e.g. ``find all frames with buses in the Taipei feed''), and constructs a model cascade exploiting difference detectors and specialized models to achieve speedups on most inputs \cite{NoScope}. Focus invokes object clustering and low-cost models to cheaply index video at ingest time, and thereby support low-latency, after-the-fact queries on historical video \cite{Focus}. Chameleon exploits correlations in camera content (e.g. velocity and sizes of detected objects) to amortize profiling costs across cameras over time \cite{Chameleon}.

This preceding work leaves three key problem areas unexplored, each of which is addressed in ReXCam.

First, all of these papers focus on single-frame analytics tasks (e.g. license plate recognition, binary frame classification, object detection), which are stateless and easily parallelized. In contrast, many real surveillance applications involve interactive or long-running queries (e.g. multi-frame tracking), where future questions are dependent on past inference results. In particular, ReXCam studies real-time tracking, a task that is difficult to parallelize or pipeline, and entails compounding classification errors (i.e. misidentifying a person at time $t$ affects all future tracking behavior).

Second, all of these papers study single-\textit{camera} analytics tasks. While some propose joint execution plans and shared profiling \cite{Optasia, Chameleon} as means to reduce redundant work, none explore the complexities involved in cross-camera inference (e.g. occlusions, perspective shifts) or collaborative execution (e.g. intermediate state sharing), a defining component of many key applications, such as person re-identification. Moreover, none model the dynamics of the camera network itself to inform future inference decisions, as ReXCam does by profiling cross-camera traffic patterns.

Third, all focus on standard classification tasks, where objects or activities of interest at inference time fall neatly into classes seen at training time. In contrast, many real security applications involve searching for new object instances (e.g. a suspicious person), or detecting highly anomalous behavior (e.g. a bomb setup), given training data skewed overwhelmingly toward negative examples. ReXCam focuses exclusively on tasks for the first type, termed \textit{instance retrieval}, on which current techniques generally achieve low precision \cite{MSMT17}. This is because, in large datasets, many detected entities tend to match against the query identity, of which there is only one or few examples, and which was likely never seen at training time. Given this property, systems level insights -- such as our observation that cameras tend to share traffic with only a small set of neighboring nodes -- can yield particularly substantial accuracy gains.

\noindent{\bf Efficient Machine Learning.} Techniques in machine learning that addresses the bandwidth, memory, and compute costs of deploying large models fall largely into two categories: (1) training-time optimizations and (2) inference-time optimizations.

Training-time optimizations can be broadly characterized as efforts to \textit{compress} accurate but expensive models. Proposed techniques include parameter and filter pruning \cite{DeepCompress, PruningFilters}, compact architecture design \cite{SqueezeNet, NIN}, knowledge distillation \cite{Distill, DoDeepCNNs, OnlineDistill}, and model specialization \cite{NoScope, Focus}. In general, these techniques are orthogonal to ReXCam, which would gain from any reduction in the inference cost or memory size of the models it deploys (e.g. re-identification).

Work on efficient inference generally aims to address a constrained optimization problem: maximize accuracy or minimize resource usage, given specific constraints on resource availability or latency (i.e. SLOs). Prior work explores resource-aware scheduling \cite{MCDNN, NestDNN}, low-latency prediction serving \cite{Clipper}, edge-cloud compute partitioning \cite{Vigil, Glimpse}, hardware-specific optimizations \cite{DeepMon, DeepEye}, and multi-tenant resource sharing \cite{Starfish, Mainstream}. Unlike these systems, ReXCam does not aim to multiplex heterogeneous models, nor does it espouse a particular compute model (e.g. mobile, edge-cloud hybrid). Instead, ReXCam entails a new approach altogether to reducing resource usage: instead of operating cheaper models, run inference on \textit{less data}. Its mechanism for doing so is to exploit spatial and temporal locality in the data source (i.e. large camera networks).

\noindent{\bf Computer Vision.} ReXCam is most closely related to computer vision literature on person re-identification and multi-target, multi-camera (MTMC) tracking. Papers in this area generally make one of three types of contributions: (1) new datasets \cite{DukeMTMC, PRW, PersonSearch, MSMT17}, (2) new neural network architectures \cite{PRW, PersonSearch, MSMT17}, or (3) new training schemes \cite{DukeFeatures, PRW, PersonSearch}.

Examples of new architectures include networks for joint detection and re-identification \cite{PRW, PersonSearch}, and networks that enable better generalization (i.e. transfer learning) to new datasets \cite{MSMT17}. Examples of new training schemes include new loss functions \cite{DukeFeatures, PersonSearch} and new data sampling techniques (e.g. hard-identity mining \cite{DukeFeatures}, confidence weighting \cite{PRW}).

In general, the vision literature does not address the inference cost of re-identification and MTMC tracking, nor does it study \textit{online} tracking (iterated re-identification), a key application of interest in real surveillance systems. While prior work has explored the use of network topology information to improve tracking accuracy, it has generally confined itself to explicitly learning epipolar geometry in offline settings with classical vision techniques \cite{Geo1, Geo2, Geo3, Geo4, Geo5}.

\noindent{\bf Visual Data Management.} A body of work also exists in the data management space on storing querying content in image and video databases. These systems explore the use of classical computer vision techniques (e.g. clustering by low-level features, such as color and texture) to index image and video efficiently, and focus on relational, historical data stores \cite{Chabot, QBIC, VDBMS, Jacob, BrowsingDB}. We build on this tradition, revisiting large-scale visual analytics in the context of \textit{cross-camera inference} on \textit{live video} with \textit{modern computer vision} (e.g. deep learning-based) \textit{techniques}, a setting that entails substantially different challenges than the target domain of older work.
